Quantifying the Prediction Uncertainty of Machine Learning Models for Individual Data

Machine learning models have exhibited exceptional results in various domains. The most prevalent approach for learning is the empirical risk minimizer (ERM), which adapts the model's weights to reduce the loss on a training set and subsequently leverages these weights to predict the label for new test data. Nonetheless, ERM makes the assumption that the test distribution is similar to the training distribution, which may not always hold in real-world situations. In contrast, the predictive normalized maximum likelihood (pNML) was proposed as a min-max solution for the individual setting where no assumptions are made on the distribution of the tested input. This study investigates pNML's learnability for linear regression and neural networks, and demonstrates that pNML can improve the performance and robustness of these models on various tasks. Moreover, the pNML provides an accurate confidence measure for its output, showcasing state-of-the-art results for out-of-distribution detection, resistance to adversarial attacks, and active learning.

==> secs/dnn_twice_universality.tex <==
\section{Twice universality}

\begin{figure*}
\begin{minipage}[h]{0.49\columnwidth}
\null
\begin{algorithm}[H]
	\caption{Deep pNML}
	\label{alg:deep_pNML}
	\begin{algorithmic}
		\State {\bfseries Input:} $z^{N}$, $x$, $\eta$, $\lambda$, $\textit{steps}_1$, $\textit{steps}_2$
		\State Initialize $\hat{\theta}_0$ randomly
		\State Train: $\hat{\theta}_{\textit{ERM}} = SGD(\hat{\theta}_0, z^N, \eta, \lambda, \textit{steps}_1)$ 
		\For {i=1 {\bfseries to} $|\mathcal{Y}|$}
		\State $z^{N+1} = z^N \bigcup (x,y=i)$
		\State $\hat{\theta}_i = \textit{SGD}(\hat{\theta}_{\textit{ERM}}, z^{N+1}, \eta, \lambda, \textit{steps}_2)$  
		\State $p_i = p_{\hat{\theta}_i}(y=i|x)$
		\EndFor
		\State $C=\sum_{i=1}^{|\mathcal{Y}|}p_i$ 
		\State $\Gamma=\log{C}$
		\For{$i=1$ {\bfseries to} $|\mathcal{Y}|$} 
		\State $q_{\textit{pNML}}(y=i)= \frac{1}{C} p_i$
		\EndFor
		\State {\bfseries Return} $q_{\textit{pNML}}$,  $\Gamma$
	\end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}[h]{0.49\columnwidth}
\null
\begin{algorithm}[H]
   \caption{Twice Universality}
   \label{alg:twice_universality}
\begin{algorithmic}
   \State {\bfseries Input:} Test sample $x$, learners $\left\{q_k\right\}_{k=1}^K$
   \For {i=1  {\bfseries to} $|\mathcal{Y}|$}
   \State $p_i = \underset{k  \in \{1,..,K \}}{\textit{max }}q_{k}(y=i|x)$
   \EndFor
   \State $C^{\textit{TU}}=\sum_{i=1}^{|\mathcal{Y}|}P_i$ 
   \For{$i=1$ {\bfseries to} $|\mathcal{Y}|$} 
   \State $q_{\textit{pNML}}^{\textit{TU}}(y=i) =  \frac{1}{C^{\textit{TU}}} p_i$
   \EndFor
   \State {\bfseries Return} $q_{\textit{pNML}}^{\textit{TU}}$
   \State 
   \State 
   \State 
   \State 
   \vspace{0.31cm}
\end{algorithmic}
\end{algorithm}
\end{minipage}
% \hfill
\end{figure*}

In many problems the best model class is unknown, and therefore being universal with respect to several model classes can improve the performance of the learner.
As part of our research, we implemented various versions of the pNML, where during the fine-tuning phase only some layers of the DNN's are updated. 
This can be seen as a nested hierarchy model class, where the richest model is the one where all the layers are updated in the fine-tuning phase, and the smallest class is that where none of them are updated and essentially the only model in the class is the ERM. 
We treat each of these variants as different classes $\{\Theta_k\}_{k=1}^K$, and evaluate their predictors, $q_k(\cdot|x)$, based on the pNML scheme in \myalgref{alg:deep_pNML}. 
Then, we executed the twice-universal algorithm described in \myalgref{alg:twice_universality} that produces the following learner: 
\begin{equation} \label{eq:twice_universal}
q^{\textit{TU}}_{\textit{pNML}}(y|z^{N},x)= 
\frac{\underset{k \in K}{\textit{max }} q_{k} (y|z^{N}, x, y)}{\sum_{y \in \mathcal{Y}}\underset{k \in K}{\textit{max }} q_{k} (y|z^{N}, x, y)}.
\end{equation}
Using the twice universal scheme, we can produce a min-max learner which has performance as good as the best learner from the various hypothesis classes.



In addition to the universality inside a model class $\Theta$, a second universality can be made regarding the index of multiple model families $\left\{\Theta_k\right\}_{k=1}^{K}$. This is the `twice universal' approach. We consider three model classes: The first class is where the fine-tuning affected only the last two layers. In the second class fine-tuning affected all layers. The third class is simply the DNN obtained after the initial training, which is the ERM.

Our next results were obtained by twice-universality over these 3 classes: For each test sample and each label, we took the maximum of the pNML probabilities over the 3 model classes. Then we normalized the probability of the test sample in order to create a valid probability assignment, as described in \myalgref{alg:twice_universality}.
\tableref{table:twice_universality} summarizes the results on CIFAR10. The twice universal predictor is better than any other class predictor in the log-loss sense. 
In addition, its accuracy is 0.92 which is as good as the 2 layer model. 

\begin{table}
\caption{\textbf{Twice Universality performance.} The performance of the pNML learners with different amount of layers that were finetuned.}
\label{table:twice_universality}
\begin{center}
\begin{tabular}{lr}
\begin{tabular}{lccc}
\toprule
Dataset & Model & Acc.  & Loss\\
\hline
\multirow{4}{*}{CIFAR10}&   0 layers    & 0.920 &  0.203 \\
                        &   2 layers    & 0.921 &  0.173 \\ 
                        &   7 layers    & 0.913 &  0.244 \\
                        &   Twice Univ. & 0.920 &  0.168 \\
\bottomrule
\end{tabular}
&
\begin{tabular}{lccc}
\toprule
Dataset & Model & Acc.  & Loss\\
\hline
\multirow{4}{*}{MNIST}  & 0 layers      & 0.930 &   0.093 \\
                        & 1 layer      & 0.937  &   0.086 \\ 
                        & 2 layers      & 0.937 &   0.085 \\
                        & Twice Univ.   & 0.950 &   0.081 \\
\bottomrule
\end{tabular}
\end{tabular}
\end{center}
\end{table}

We also examined the twice universality method on MNIST dataset \citep{lecun-mnisthandwrittendigit-2010}. 
The network used was a simple multilayer perceptron \citep{orhan2011eeg}, with 10 hidden units. 
The initial training consisted of 100 epochs with a learning rate of 0.01 for the first 10 epochs, 0.01 for the next 30, 0.001 for the next 40 and 0.0001 for the rest. 
Next, we executed the pNML procedure of \myalgref{alg:deep_pNML}. 
The fine-tuning phase consisted of 10 epochs with a learning rate of 0.0001, changing either the two layers or only the last one.
The results of the twice universality method on MNIST dataset are also presented in \tableref{table:twice_universality}. 
The twice universal learner has the best performance, both in the log-loss and the accuracy rate. Since this learner is close to the optimal one for every specific sample, it seems that it avoids the pitfalls of each of the other learners and thus manages to outperform them.

==> secs/ordinary_least_squares_bayesian.tex <==
\subsection{Bayesian linear regression}
In Bayesian prediction, to perform a prediction we compute a mean over all plausible parameters settings (according to the posterior)~\cite{deisenroth2020mathematics}. We define, for example, a Gaussian prior 
\begin{equation}
    p(\theta) = \mathcal{N}(m_0, S_0)
\end{equation}
which turns the parameter vector into a random variable.
To perform a prediction for a test vector $x$, we average over all plausible parameter setting according to the prior distribution
\begin{equation}
    p(y|x) = \int p(y|x,\theta) p(\theta) d\theta.
\end{equation}
Using the Gaussian prior, the predictive distribution is
\begin{equation}
    p(y|x) = \mathcal{N}\left(x^\top m_0, x^\top S_0 x + \sigma^2 \right)
\end{equation}

To compute the predictive distribution with the posterior distribution (instead of the prior), we replace $p(\theta)$ with $p(\theta|D_N)$ which is
\begin{equation}
    p(\theta|D_N) = \mathcal{N} \left(\theta^\top m_N, S_N\right)
\end{equation}
where 
\begin{equation}
S_N = \left(S_0^{-1} + \sigma^{-2} X_N^\top X_N \right)^{-1}, \quad m_N = S_N \left(S_0^{-1} m_0 + \sigma^{-2} X_N^\top Y_N \right)
\end{equation}
The (posterior) predictive distribution is
\begin{equation}
\begin{split}
    p(y|x,D_N) &= \int p(y|x,\theta)p(\theta|D_N) d\theta 
    = 
    \mathcal{N} \left(x^\top m_N, x^\top S_N x + \sigma^2  \right).
\end{split}
\end{equation}
The prediction uncertainty is encoded in $x^\top S_N x$. The prediction mean $x^\top m_N$ is equivalent to the MAP estimator.

When $m_0=0$ and $S_0 = \lambda \sigma^{-2} I$ we get
\begin{equation}
\begin{split}
    S_N &= \sigma^2 \left(X_N^\top X_N + \lambda I \right)^{-1} \\
    m_N &= S_N \sigma^{-2} X_N^\top Y_N =  \left(X_N^\top X_N + \lambda I \right)^{-1}X_N^\top Y_N
\end{split}
\end{equation}
such the the prediction $x_N^\top m_N$ coincide ride regression prediction. The predictive variance is $\hat{\sigma}^2 =\sigma^2\left(1+ x^\top \left(X_N^\top X_N + \lambda I \right)^{-1}  x \right)$

pNML and Bayesian regression


LpNML and Bayesian regression. With noise $\sigmalpnml=x^\top S_N x + \sigma^2$
\begin{equation}
\frac{\sigma^2 \Klamb^2}{1+\lambda x^\top \Plamb^2 x} = x^\top \left(S_0^{-1} + \sigma^{-2} X_N^\top X_N \right)^{-1} x + \sigma^2
\end{equation}
Setting $S_0 = \sigma^2 S_0'$
\begin{equation}
\frac{\left(1 + x^\top \Plamb x\right)^2}{1+\lambda x^\top \Plamb^2 x} = 1 + x^\top \left(S_0'^{-1} + X_N^\top X_N \right)^{-1} x 
\end{equation}
\begin{equation}
\frac{\left(1 + x^\top \Plamb x\right)^2 - 1 - \lambda x^\top \Plamb^2 x}{1+\lambda x^\top \Plamb^2 x} =  x^\top \left(S_0'^{-1} + X_N^\top X_N \right)^{-1} x 
\end{equation}
\begin{equation}
\frac{2  x^\top \Plamb x +  (x^\top \Plamb x)^2 - \lambda x^\top \Plamb^2 x}{1+\lambda x^\top \Plamb^2 x} =  x^\top \left(S_0'^{-1} + X_N^\top X_N \right)^{-1} x 
\end{equation}
\begin{equation}
x^\top \frac{2  \Plamb +  \Plamb x x^\top \Plamb - \lambda \Plamb^2}{1+\lambda x^\top \Plamb^2 x} x =  x^\top \left(S_0'^{-1} + X_N^\top X_N \right)^{-1} x 
\end{equation}
So we need to find $S_0'$ such that
\begin{equation}
\frac{2  \Plamb +  \Plamb x x^\top \Plamb - \lambda \Plamb^2}{1+\lambda x^\top \Plamb^2 x} =  \left(S_0'^{-1} + X_N^\top X_N \right)^{-1} 
\end{equation}
\begin{equation}
\left(1+\lambda x^\top \Plamb^2 x\right)
\left(2  \Plamb +  \Plamb x x^\top \Plamb - \lambda \Plamb^2 \right)^{-1} =  S_0'^{-1} + X_N^\top X_N 
\end{equation}
\begin{equation}
\begin{split}
 S_0'^{-1}  &= 
\left(1+\lambda x^\top \Plamb^2 x\right)
\left(2  \Plamb +  \Plamb x x^\top \Plamb - \lambda \Plamb^2 \right)^{-1} - X_N^\top X_N 
\\  &=
\left(1+\lambda x^\top \Plamb^2 x\right)
\left(\Plamb \left[2 \Plamb^{-1} +  x x^\top - \lambda I \right] \Plamb\right)^{-1} - X_N^\top X_N 
\\  &=
\left(1+\lambda x^\top \Plamb^2 x\right)
\left(\Plamb \left[2 \left(X_N^\top X_N + \lambda I\right) +  x x^\top - \lambda I \right] \Plamb\right)^{-1} - X_N^\top X_N 
\\  &=
\left(1+\lambda x^\top \Plamb^2 x\right)
\left(\Plamb \left[2 X_N^\top X_N + \lambda I +  x x^\top \right] \Plamb\right)^{-1} - X_N^\top X_N
\\  &=
\left(1+\lambda x^\top \Plamb^2 x\right)
\Plamb^{-1} \left[2 X_N^\top X_N + \lambda I +  x x^\top \right]^{-1} \Plamb^{-1} - X_N^\top X_N
\\  &=
\left(1+\lambda x^\top \Plamb^2 x\right)
\Plamb^{-1} 
\left[\left(2 X_N^\top X_N + \lambda I\right)^{-1} - \frac{\left(2 X_N^\top X_N + \lambda I\right)^{-1}x x^\top \left(2 X_N^\top X_N + \lambda I\right)^{-1}}{1 + x^\top \left(2 X_N^\top X_N + \lambda I\right)^{-1} x}\right]
\Plamb^{-1} - X_N^\top X_N
\end{split}
\end{equation}

==> secs/preliminaries.tex <==
\section{Universal learning}

\section{The pNML derivation}
In the supervised machine learning scenario, a training set consisting of $N$ pairs of examples is given
\begin{equation}
\mathcal{D}_N = \{(x_n,y_n)\}_{n=1}^{N}, \quad x_n \in {\cal X}, \quad y_n \in {\cal Y},
\end{equation}
where $x_n$ is the $n$-th data instance and $y_n$ is its corresponding label.
The goal of a learner is to predict the unknown test label $y$ given a new test data $x$ by assigning probability distribution $q(\cdot|x)$ to the unknown label. 
The performance is evaluated using the log-loss function
\begin{equation} \label{eq:logloss}
   \ell(q;x,y) = -\log {q(y|x)}.
\end{equation}

For the problem to be well-posed, we must make further assumptions on the class of possible models or {\em hypothesis set} that is used to find the relation between $x$ and $y$.
Denote $\Theta$ as a general index set, this class is a set of conditional probability distributions 
\begin{equation} \label{eq:hypotesis_set}
P_\Theta = \{p_\theta(y|x),\;\;\theta\in\Theta\}.
\end{equation}
The ERM is the learner from the hypothesis set that attains the minimal log-loss on the training set.





==> tables/linear_regression_with_luckiness/uci_meta_data.tex <==
\begin{tabular}{l c c c}
\toprule
% Dataset name & Dataset size & Feature number \\
Dataset name & $N$ & $M$ & \#Splits\\
\midrule
Boston Housing & 506 & 13 & 20 \\
Concrete Strength & 1,030 & 8 & 20 \\ % Concrete Compression Strength
Energy Efficiency & 768 & 8 & 20 \\
Kin8nm & 8,192 & 8 & 20 \\
Naval Propulsion & 11,934 & 16 & 20\\
Cycle Power Plant & 9,568 & 4 & 20\\ % Combined Cycle Power Plant
Protein Structure & 45,730 & 9  & 5 \\
Wine Quality Red & 1599 & 11 & 20\\
Yacht Hydrodynamics & 308 & 6 & 20\\
% Year Prediction MSD & 515,345 & 90 \\
\bottomrule % thead
\end{tabular}
